Lattice Knots in a Slab

In this paper the number and lengths of minimal length lattice knots confined to slabs of width $L$, is determined. Our data on minimal length verify the results by Sharein et.al. (2011) for the similar problem, expect in a single case, where an improvement is found. From our data we construct two models of grafted knotted ring polymers squeezed between hard walls, or by an external force. In each model, we determine the entropic forces arising when the lattice polygon is squeezed by externally applied forces. The profile of forces and compressibility of several knot types are presented and compared, and in addition, the total work done on the lattice knots when it is squeezed to a minimal state is determined.

==> Bargraphs/Bargraph3-1k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,124.267 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 1.609 1.000 1.609 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 1.609 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 1.236 2.000 1.236 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 1.236 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 1.221 3.000 1.221 3.000 0.000   /

 \color{red}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 1.221 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 0.002 4.000 0.002 4.000 0.000   /

\plot 4.000 0.000 4.000 0.000 5.000 0.000 5.000 0.000   /

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,124.267 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 1.609438
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 1.2 4.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph4-1k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,70.591 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 2.833 1.000 2.833 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 2.833 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 2.343 2.000 2.343 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 2.343 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 0.181 3.000 0.181 3.000 0.000   /

 \color{blue}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 0.181 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 0.257 4.000 0.257 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 0.257 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.000 5.000 0.000 5.000 0.000   /

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,70.591 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 2.833213
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 3.1 16.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph5-1k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,80.486 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 2.485 1.000 2.485 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 2.485 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 1.996 2.000 1.996 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 1.996 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 0.459 3.000 0.459 3.000 0.000   /

 \color{red}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 0.459 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 0.634 4.000 0.634 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 0.634 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.012 5.000 0.012 5.000 0.000   /

 \color{red}
\setshadegrid span <1.462009pt>
\hshade 0.000 4.000 5.000 0.012 4.000 5.000  /

 \color{red}

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,80.486 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 2.484907
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 2.5 11.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph5-2k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,80.486 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 2.485 1.000 2.485 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 2.485 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 2.059 2.000 2.059 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 2.059 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 1.513 3.000 1.513 3.000 0.000   /

 \color{red}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 1.513 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 0.589 4.000 0.589 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 0.589 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.037 5.000 0.037 5.000 0.000   /

 \color{red}
\setshadegrid span <1.462009pt>
\hshade 0.000 4.000 5.000 0.037 4.000 5.000  /

 \color{red}

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,80.486 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 2.484907
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 2.5 11.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph6-1k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,61.386 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 3.258 1.000 3.258 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 3.258 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 2.801 2.000 2.801 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 2.801 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 -0.870 3.000 -0.870 3.000 0.000   /

\plot 3.000 0.000 3.000 0.664 4.000 0.664 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 0.664 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.023 5.000 0.023 5.000 0.000   /

 \color{red}
\setshadegrid span <1.462009pt>
\hshade 0.000 4.000 5.000 0.023 4.000 5.000  /

 \color{red}

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,61.386 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 3.258097
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 4.1 25.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph6-2k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,62.932 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 3.178 1.000 3.178 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 3.178 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 2.700 2.000 2.700 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 2.700 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 1.230 3.000 1.230 3.000 0.000   /

 \color{blue}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 1.230 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 0.952 4.000 0.952 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 0.952 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.109 5.000 0.109 5.000 0.000   /

 \color{red}
\setshadegrid span <1.462009pt>
\hshade 0.000 4.000 5.000 0.109 4.000 5.000  /

 \color{red}

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,62.932 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 3.178054
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 3.9 23.0 / quantity 3 / 
\normalcolor
\endpicture


==> Bargraphs/Bargraph6-3k1L.tex <==
\beginpicture

 \setcoordinatesystem units <30.000 pt,54.982 pt>


 \color{red}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0.000 0.000 0.000 3.638 1.000 3.638 1.000 0.000   /

 \color{blue}
\setshadegrid span <0.500000pt>
\hshade 0.000 0.000 1.000 3.638 0.000 1.000  /

 \color{red}

\plot 1.000 0.000 1.000 3.170 2.000 3.170 2.000 0.000   /

 \color{blue}
\setshadegrid span <0.793701pt>
\hshade 0.000 1.000 2.000 3.170 1.000 2.000  /

 \color{red}

\plot 2.000 0.000 2.000 0.899 3.000 0.899 3.000 0.000   /

 \color{blue}
\setshadegrid span <1.040042pt>
\hshade 0.000 2.000 3.000 0.899 2.000 3.000  /

 \color{red}

\plot 3.000 0.000 3.000 1.012 4.000 1.012 4.000 0.000   /

 \color{red}
\setshadegrid span <1.259921pt>
\hshade 0.000 3.000 4.000 1.012 3.000 4.000  /

 \color{red}

\plot 4.000 0.000 4.000 0.041 5.000 0.041 5.000 0.000   /

 \color{red}
\setshadegrid span <1.462009pt>
\hshade 0.000 4.000 5.000 0.041 4.000 5.000  /

 \color{red}

\plot 5.000 0.000 5.000 0.000 6.000 0.000 6.000 0.000   /

\plot 6.000 0.000 6.000 0.000 7.000 0.000 7.000 0.000   /

\plot 7.000 0.000 7.000 0.000 8.000 0.000 8.000 0.000   /

\plot 8.000 0.000 8.000 0.000 9.000 0.000 9.000 0.000   /

\plot 9.000 0.000 9.000 0.000 10.000 0.000 10.000 0.000   /

 \setcoordinatesystem units <30.000 pt,54.982 pt>


 \color{black}
\put {O} at 0 0 
\setplotarea x from 0 to 10.000000, y from 0 to 3.637586
\axis top /
\axis right /
\axis bottom 
 label {{\Large \hspace{2.7cm} $L$}} /
\axis bottom 
 ticks numbered from 0 to 10 by 1 /
\axis left 
 label {{\Large $Force \hbox{$\qquad$}$}} /
\axis left 
 ticks withvalues 0 5.2 37.0 / quantity 3 / 
\normalcolor
\endpicture

